Virtual concordance and the generalized Alexander polynomial

We use the Bar-Natan Zh-correspondence to identify the generalized Alexander polynomial of a virtual knot with the Alexander polynomial of a two component welded link. We show that the Zh-map is functorial under concordance, and also that Satoh's Tube map (from welded links to ribbon knotted tori in $S^4$) is functorial under concordance. In addition, we extend classical results of Chen, Milnor, and Hillman on the lower central series of link groups to links in thickened surfaces. Our main result is that the generalized Alexander polynomial vanishes on any knot in a thickened surface which is concordant to a homologically trivial knot. In particular, this shows that it vanishes on virtually slice knots. We apply it to complete the calculation of the slice genus for virtual knots with four crossings and to determine non-sliceness for a number of 5-crossing and 6-crossing virtual knots.

==> Figures/mpxerr.tex <==
\gdef\mpxshipout{\shipout\hbox\bgroup
  \setbox0=\hbox\bgroup}
\gdef\stopmpxshipout{\egroup  \dimen0=\ht0 \advance\dimen0\dp0
  \dimen1=\ht0 \dimen2=\dp0
  \setbox0=\hbox\bgroup
    \box0
    \ifnum\dimen0>0 \vrule width1sp height\dimen1 depth\dimen2 
    \else \vrule width1sp height1sp depth0sp\relax
    \fi\egroup
  \ht0=0pt \dp0=0pt \box0 \egroup}
\mpxshipout% line 30 ./crossing-reg.mp
$a_{k\ell}$%
\stopmpxshipout
\mpxshipout% line 31 ./crossing-reg.mp
$a_{ij}$%
\stopmpxshipout
\mpxshipout% line 32 ./crossing-reg.mp
$a_{ij+1}$%
\stopmpxshipout
\mpxshipout% line 33 ./crossing-reg.mp
$\varepsilon_{ij} = 1$%
\stopmpxshipout
\mpxshipout% line 46 ./crossing-reg.mp
$a_{ij$%
\stopmpxshipout
\mpxshipout% line 47 ./crossing-reg.mp
$a_{k\ell}$%
\stopmpxshipout
\mpxshipout% line 48 ./crossing-reg.mp
$a_{ij+1}$%
\stopmpxshipout
\mpxshipout% line 49 ./crossing-reg.mp
$\varepsilon_{ij} = -1$%
\stopmpxshipout
\end{document}

